Federated Learning in UAV-Enhanced Networks: Joint Coverage and Convergence Time Optimization

Federated learning (FL) involves several devices that collaboratively train a shared model without transferring their local data. FL reduces the communication overhead, making it a promising learning method in UAV-enhanced wireless networks with scarce energy resources. Despite the potential, implementing FL in UAV-enhanced networks is challenging, as conventional UAV placement methods that maximize coverage increase the FL delay significantly. Moreover, the uncertainty and lack of a priori information about crucial variables, such as channel quality, exacerbate the problem. In this paper, we first analyze the statistical characteristics of a UAV-enhanced wireless sensor network (WSN) with energy harvesting. We then develop a model and solution based on the multi-objective multi-armed bandit theory to maximize the network coverage while minimizing the FL delay. Besides, we propose another solution that is particularly useful with large action sets and strict energy constraints at the UAVs. Our proposal uses a scalarized best-arm identification algorithm to find the optimal arms that maximize the ratio of the expected reward to the expected energy cost by sequentially eliminating one or more arms in each round. Then, we derive the upper bound on the error probability of our multi-objective and cost-aware algorithm. Numerical results show the effectiveness of our approach.

==> bibliography.tex <==
@ARTICLE{zhang2022,
  author={Zhang, Zhe and Ma, Shiyao and Yang, Zhaohui and Xiong, Zehui and Kang, Jiawen and Wu, Yi and Zhang, Kejia and Niyato, Dusit},
  journal={IEEE Internet of Things J.}, 
  title={Robust Semi-supervised Federated Learning for Images Automatic Recognition in Internet of Drones}, 
  year={2022},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/JIOT.2022.3151945}}
%------------------------------------------------  
@article{nguyen2021federated,
  title={Federated learning for internet of things: A comprehensive survey},
  author={Nguyen, Dinh C and Ding, Ming and Pathirana, Pubudu N and Seneviratne, Aruna and Li, Jun and Poor, H Vincent},
  journal={IEEE Commun. Surv. \& Tut.},
  volume={23},
  number={3},
  pages={1622--1658},
  year={2021},
  publisher={IEEE}
}  
%---------------------------------------------------
@ARTICLE{FL_Brik2020,
author={B. {Brik} and A. {Ksentini} and M. {Bouaziz}},
journal={IEEE Access}, 
title={Federated Learning for {UAVs}-Enabled Wireless Networks: Use Cases, Challenges, and Open Problems}, 
year={2020},
volume={8},
number={},
pages={53841-53849}}
%-----------------------------------------------
@INPROCEEDINGS{FL_zeng2020,  
author={T. {Zeng} and O. {Semiari} and M. {Mozaffari} and M. {Chen} and W. {Saad} and M. {Bennis}},  
booktitle={Proc. Int. Conf. Commun. (ICC)},  
title={Federated Learning in the Sky: Joint Power Allocation and Scheduling with {UAV} Swarms},   
year={2020},  
pages={1-6},  
}
%--------------------------------------------
@article{yang2021privacy,
  title={Privacy-preserving federated learning for {UAV}-enabled networks: Learning-based joint scheduling and resource management},
  author={Yang, Helin and Zhao, Jun and Xiong, Zehui and Lam, Kwok-Yan and Sun, Sumei and Xiao, Liang},
  journal={IEEE J. on Sel. Areas in Commun.},
  volume={39},
  number={10},
  pages={3144--3159},
  year={2021},
  publisher={IEEE}
}
%---------------------------------------------------------
@article{chen2020convergence,
  title={Convergence time optimization for federated learning over wireless networks},
  author={Chen, Mingzhe and Poor, H Vincent and Saad, Walid and Cui, Shuguang},
  journal={IEEE Trans. on Wireless Commun.},
  volume={20},
  number={4},
  pages={2457-2471},
  year={2020},
  publisher={IEEE}
}
%---------------------------------------------------------
@ARTICLE{FL_Dinh2021,
    author={C. {Dinh} and N. {Tran} and M. {Nguyen} and C. {Hong} and W. {Bao} and A. {Zomaya} and V. {Gramoli}},
    journal={IEEE/ACM Trans. on Netw.}, title={Federated Learning Over Wireless Networks: Convergence Analysis and Resource Allocation}, 
    year={2021},
    volume={29},
    number={1},
    pages={398-409}}
%-----------------------------------------------------------
@INPROCEEDINGS{yahya2022,  
    author={M. {Yahya} and S. {Maghsudi}},  
    booktitle={Proc. IEEE Wireless Commun. Netw. Conf. (WCNC)},   
    title={Joint coverage and resource allocation for federated learning in {UAV}-enabled networks},   
    year={2022},  
    pages={1-6},  
    }
%-----------------------------------------------------------
@INPROCEEDINGS{drugan2013,
    author={Drugan, Madalina M. and Nowe, Ann},
    booktitle={The 2013 Int. Joint Conf. on Neural Netw. (IJCNN)},
    title={Designing multi-objective multi-armed bandits algorithms: A study},
    year={2013},
    volume={},
    number={},
    pages={1-8},
    doi={10.1109/IJCNN.2013.6707036}
    }
%-------------------------------------------------------
@ARTICLE{Maghsudi16:MAB,
  author={Maghsudi, S. and Hossain, E.},
  journal={IEEE Wireless Commun.}, 
  title={Multi-armed bandits with application to {5G} small cells}, 
  year={2016},
  volume={23},
  number={3},
  pages={64-73},
  doi={10.1109/MWC.2016.7498076}}
%-------------------------------------------------------
@article{ruadulescu2020,
  title={Multi-objective multi-agent decision making: {A} utility-based analysis and survey},
  author={R{\u{a}}dulescu, Roxana and Mannion, Patrick and Roijers, Diederik M and Now{\'e}, Ann},
  journal={Auton. Agents and Multi-Agent Syst.},
  volume={34},
  number={1},
  pages={1-52},
  year={2020},
  publisher={Springer}
}
%-------------------------------------------------------
@inproceedings{audibert2010best,
  title={Best arm identification in multi-armed bandits.},
  author={Audibert, Jean-Yves and Bubeck, S{\'e}bastien and Munos, R{\'e}mi},
  booktitle={COLT},
  pages={41--53},
  year={2010},
  organization={Citeseer}
}
%-------------------------------------------------------
@article{shahrampour2017sequential,
  title={On sequential elimination algorithms for best-arm identification in multi-armed bandits},
  author={Shahrampour, Shahin and Noshad, Mohammad and Tarokh, Vahid},
  journal={IEEE Trans. on Signal Process.},
  volume={65},
  number={16},
  pages={4281--4292},
  year={2017},
  publisher={IEEE}
}
%--------------------------------------------------------
@inproceedings{drugan2014scalarization,
  title={Scalarization based {P}areto optimal set of arms identification algorithms},
  author={Drugan, Madalina M and Now{\'e}, Ann},
  booktitle={2014 Int. Joint Conf. on Neural Netw. (IJCNN)},
  pages={2690--2697},
  year={2014},
  organization={IEEE}
}
%-------------------------------------------
@article{maghsudi2017distributed,
  title={Distributed user association in energy harvesting small cell networks: A probabilistic bandit model},
  author={Maghsudi, Setareh and Hossain, Ekram},
  journal={IEEE Trans. on Wireless Commun.},
  volume={16},
  number={3},
  pages={1549--1563},
  year={2017},
  publisher={IEEE}
}
%------------------------------------------------------------
@book{balanis2015,
  title={Antenna Theory: Analysis and Design},
  author={Balanis, Constantine A},
  year={2015},
  publisher={John wiley \& sons}
}
%------------------------------------------------------------
@ARTICLE{alhourani2014,  
    author={A. {Al-Hourani} and S. {Kandeepan} and S. {Lardner}},  
    journal={IEEE Wireless Commun. Lett.}, 
    title={Optimal {LAP} Altitude for Maximum Coverage},  
    year={2014},  
    volume={3},  
    number={6},  
    pages={569-572},  
}
%------------------------------------------------------------
@book{john2008digital,
  title={Digital Communications},
  author={John G.. Proakis and Salehi, Masoud},
  publisher={McGraw-Hill.},
  year={2008},
}
%------------------------------------------------------------
@book{papoulis02,
  added-at = {2015-10-23T15:50:51.000+0200},
  address = {Boston},
  author = {Papoulis, Athanasios and Pillai, S.},
  biburl = {https://www.bibsonomy.org/bibtex/22a938c6a45a64bd0f43a8ebbf1f3e368/ytyoun},
  edition = {4th},
  interhash = {da558c64a1da0ca6035c9f1766b0c15b},
  intrahash = {2a938c6a45a64bd0f43a8ebbf1f3e368},
  isbn = {0071122567 9780071122566 0073660116 9780073660110 0071226613 9780071226615},
  keywords = {probability textbook},
  publisher = {McGraw Hill},
  refid = {611571290},
  timestamp = {2015-10-23T15:50:51.000+0200},
  title = {Probability, Random Variables, and Stochastic Processes},
  url = {http://www.worldcat.org/search?qt=worldcat_org_all&q=0071226613},
  year = 2002
}
%--------------------------------------------------------------
@book{arnold2008first,
  title={A First Course in Order Statistics},
  author={Arnold, Barry C and Balakrishnan, Narayanaswamy and Nagaraja, Haikady Navada},
  year={2008},
  publisher={SIAM}
}
%--------------------------------------------------------------
@article{xia2020multi,
  title={Multi-armed bandit-based client scheduling for federated learning},
  author={Xia, Wenchao and Quek, Tony QS and Guo, Kun and Wen, Wanli and Yang, Howard H and Zhu, Hongbo},
  journal={IEEE Trans. on Wireless Commun.},
  volume={19},
  number={11},
  pages={7108--7123},
  year={2020},
  publisher={IEEE}
}
%-------------------------------------------------------------
@ARTICLE{Huang2021,
  author={Huang, Tiansheng and Lin, Weiwei and Wu, Wentai and He, Ligang and Li, Keqin and Zomaya, Albert Y.},
  journal={IEEE Trans. on Parallel and Distrib. Syst.}, 
  title={An Efficiency-Boosting Client Selection Scheme for Federated Learning With Fairness Guarantee}, 
  year={2021},
  volume={32},
  number={7},
  pages={1552-1564},
  doi={10.1109/TPDS.2020.3040887}}
%----------------------------------------------------------------
@inproceedings{cho2020bandit,
  title={Bandit-based communication-efficient client selection strategies for federated learning},
  author={Cho, Yae Jee and Gupta, Samarth and Joshi, Gauri and Ya{\u{g}}an, Osman},
  booktitle={2020 54th Asilomar Conf. on Signals, Syst., and Comput.},
  pages={1066--1069},
  year={2020},
  organization={IEEE}
}
%---------------------------------------------------------------
@article{xia2021federated,
  title={Federated-learning-based client scheduling for low-latency wireless communications},
  author={Xia, Wenchao and Wen, Wanli and Wong, Kai-Kit and Quek, Tony QS and Zhang, Jun and Zhu, Hongbo},
  journal={IEEE Wireless Commun.},
  volume={28},
  number={2},
  pages={32--38},
  year={2021},
  publisher={IEEE}
}
%---------------------------------------------------------------
@ARTICLE{9390199,
  author={Xu, Bo and Xia, Wenchao and Zhang, Jun and Quek, Tony Q. S. and Zhu, Hongbo},
  journal={IEEE Wireless Commun. Letters}, 
  title={Online Client Scheduling for Fast Federated Learning}, 
  year={2021},
  volume={10},
  number={7},
  pages={1434-1438},
  doi={10.1109/LWC.2021.3069541}}
%-------------
@inproceedings{becking2022adaptive,
  title={Adaptive Differential Filters for Fast and Communication-Efficient Federated Learning},
  author={Becking, Daniel and Kirchhoffer, Heiner and Tech, Gerhard and Haase, Paul and M{\"u}ller, Karsten and Schwarz, Heiko and Samek, Wojciech},
  booktitle={Proc. of the IEEE/CVF Conf. on Comput. Vision and Pattern Recognit.},
  pages={3367--3376},
  year={2022}
}
%--------------------------------------
@inproceedings{mcmahan2017communication,
  title={Communication-efficient learning of deep networks from decentralized data},
  author={McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and y Arcas, Blaise Aguera},
  booktitle={Artif. Intell. and Statist.},  publisher={PMLR},
  pages={1273--1282},
  year={2017}
}
%--------------------------------------
@article{zhang2021clien,
  title={Client selection for federated learning with non-iid data in mobile edge computing},
  author={Zhang, Wenyu and Wang, Xiumin and Zhou, Pan and Wu, Weiwei and Zhang, Xinglin},
  journal={IEEE Access},
  volume={9},
  pages={24462--24474},
  year={2021},
  publisher={IEEE}
}
%--------------------------------------------
 @article{he2017joint,
  title={Joint altitude and beamwidth optimization for {UAV}-enabled multiuser communications},
  author={He, Haiyun and Zhang, Shuowen and Zeng, Yong and Zhang, Rui},
  journal={IEEE Commun. Lett.},
  volume={22},
  number={2},
  pages={344--347},
  year={2017},
  publisher={IEEE}
}
%--------------------------
@article{zhang2021client,
  title={Client selection for federated learning with non-iid data in mobile edge computing},
  author={Zhang, Wenyu and Wang, Xiumin and Zhou, Pan and Wu, Weiwei and Zhang, Xinglin},
  journal={IEEE Access},
  volume={9},
  pages={24462--24474},
  year={2021},
  publisher={IEEE}
}
%-----------------------------
@article{yang2019energy,
  title={Energy efficient resource allocation in {UAV}-enabled mobile edge computing networks},
  author={Yang, Zhaohui and Pan, Cunhua and Wang, Kezhi and Shikh-Bahaei, Mohammad},
  journal={IEEE Trans. on Wireless Commun.},
  volume={18},
  number={9},
  pages={4576--4589},
  year={2019},
  publisher={IEEE}
}
%----------------------------------
@article{grossi2021energy,
  title={Energy harvesting strategies for wireless sensor networks and mobile devices: {A} review},
  author={Grossi, Marco},
  journal={Electronics},
  volume={10},
  number={6},
  pages={661},
  year={2021},
  publisher={MDPI}
}
%----------------
@inproceedings{xia2016best,
  title={Best action selection in a stochastic environment},
  author={Xia, Yingce and Qin, Tao and Yu, Nenghai and Liu, Tie-Yan},
  booktitle={Proc. of the 2016 Int. Conf. on Auton. Agents \& Multiagent Syst.},
  pages={758--766},
  year={2016}
}
%--------------------------------
@INPROCEEDINGS{yahya_conf,
  author={Yahya, Mariam and Maghsudi, Setareh and Stanczak, Slawomir},
  booktitle={Eur. Wireless 2022: 27th Eur. Wireless Conf.}, 
  title={Federated Learning in {UAV}-Enhanced Networks: Joint Coverage and Convergence Time Optimization}, 
  year={2022},
  volume={},
  number={},
  pages={1-7},
  doi={}}
%----------------
@incollection{deb2011multi,
  title={Multi-objective optimisation using evolutionary algorithms: {A}n introduction},
  author={Deb, Kalyanmoy},
  booktitle={Multi-objective Evol. Optim. for Product Des. and Manuf.},
  pages={3--34},
  year={2011},
  publisher={Springer}
}
%------------------------
@article{yang2021fresh,
  title={Fresh, fair and energy-efficient content provision in a private and cache-enabled UAV network},
  author={Yang, Peng and Guo, Kun and Xi, Xing and Quek, Tony QS and Cao, Xianbin and Liu, Chenxi},
  journal={IEEE J. of Sel. Topics in Signal Process.},
  volume={16},
  number={1},
  pages={97--112},
  year={2021},
  publisher={IEEE}
}
%------------------------
@article{yang2021proactive,
  title={Proactive {UAV} network slicing for {URLLC} and mobile broadband service multiplexing},
  author={Yang, Peng and Xi, Xing and Guo, Kun and Quek, Tony QS and Chen, Jingxuan and Cao, Xianbin},
  journal={IEEE J. on Sel. Areas in Commun.},
  volume={39},
  number={10},
  pages={3225--3244},
  year={2021},
  publisher={IEEE}
}
%-------------------------
@article{peng2023energy,
  title={Energy harvesting reconfigurable intelligent surface for {UAV} based on robust deep reinforcement learning},
  author={Peng, Haoran and Wang, Li-Chun},
  journal={IEEE Trans. on Wireless Commun.},
  year={2023},
  publisher={IEEE}
}
%--------------------------
@ARTICLE{lan2023uav,
  author={Lan, Xunqiang and Tang, Xiao and Zhang, Ruonan and Lin, Wensheng and Han, Zhu},
  journal={IEEE Wireless Commun. Lett.}, 
  title={{UAV}-Assisted Computation Offloading Toward Energy-Efficient Blockchain Operations in Internet of Things}, 
  year={2023},
  volume={12},
  number={8},
  pages={1469-1473},
  doi={10.1109/LWC.2023.3279317}}
%-------------------------
@book{miettinen1999nonlinear,
  title={Nonlinear {M}ultiobjective {O}ptimization},
  author={Miettinen, Kaisa},
  year={1999},
  publisher={Springer Science \& Business Media}
}
%------------------
@article{friha2021internet,
  title={Internet of things for the future of smart agriculture: A comprehensive survey of emerging technologies},
  author={Friha, Othmane and Ferrag, Mohamed Amine and Shu, Lei and Maglaras, Leandros and Wang, Xiaochan},
  journal={IEEE/CAA J. of Automatica Sinica},
  volume={8},
  number={4},
  pages={718--752},
  year={2021},
  publisher={IEEE/CAA Journal of Automatica Sinica}
}
%---------
@INPROCEEDINGS{9500804,
  author={Cao, Yuwen and Maghsudi, Setareh and Ohtsuki, Tomoaki},
  booktitle={ICC 2021 - IEEE Int. Conf. Commun}, 
  title={Mobility-Aware Routing and Caching: A Federated Learning Assisted Approach}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/ICC42927.2021.9500804}}
%-----------------
@ARTICLE{10044185,
  author={Balef, Amir Rezaei and Maghsudi, Setareh},
  journal={IEEE Wireless Commun. Lett.}, 
  title={Piecewise-Stationary Multi-Objective Multi-Armed Bandit With Application to Joint Communications and Sensing}, 
  year={2023},
  volume={12},
  number={5},
  pages={809-813},
  doi={10.1109/LWC.2023.3244686}}
